MatryODShka: Real-time 6DoF Video View Synthesis using Multi-Sphere Images

We introduce a method to convert stereo 360{\deg} (omnidirectional stereo) imagery into a layered, multi-sphere image representation for six degree-of-freedom (6DoF) rendering. Stereo 360{\deg} imagery can be captured from multi-camera systems for virtual reality (VR), but lacks motion parallax and correct-in-all-directions disparity cues. Together, these can quickly lead to VR sickness when viewing content. One solution is to try and generate a format suitable for 6DoF rendering, such as by estimating depth. However, this raises questions as to how to handle disoccluded regions in dynamic scenes. Our approach is to simultaneously learn depth and disocclusions via a multi-sphere image representation, which can be rendered with correct 6DoF disparity and motion parallax in VR. This significantly improves comfort for the viewer, and can be inferred and rendered in real time on modern GPU hardware. Together, these move towards making VR video a more comfortable immersive medium.

==> src/4-fig-grandcanyon1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Image results - Scene 3 Grand Canyon 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[tp]
	%
    \newcommand{\gcy}{/novel-view-sequence/gcy/}
    \newcommand{\gcyBaseline}{/novel-view-sequence/gcy/doubleplane_odsods/}
    %
    % We need two center environments because, for some reason, '\centering' or a single center environment does not produce the right result.
	\begin{center} 
	\begin{tikzpicture}[
	image/.style={inner sep=0pt, outer sep=0pt},
	collabel/.style={above=9pt, anchor=north, inner ysep=0pt, scale=0.8, align=center},
	rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
	subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
	arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
	]

	\def\padding{0.005\linewidth}
	\newcommand{\subfig}[2][0px 0px 0px 0px]{\includegraphics[width=0.25\linewidth, trim=#1, clip]{figures/#2.png}}
	\newcommand{\subbig}[2][0px 0px 0px 0px]{\includegraphics[width=0.49\linewidth, height=0.3675\linewidth, trim=#1, clip]{figures/#2.png}}
	
	%% Result 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%% Top row :: ODS input + pseudodepth + new view
	\node [image,below=20pt]                       (result1-ods-l) at (result1-blend3.south)     {\subfig{\gcy/ref_image_video1_grandcanyonsequence1_0066_010}};
	\node [image,right=\padding]                   (result1-ods-r) at (result1-ods-l.east)       {\subfig{\gcy/src_image_video1_grandcanyonsequence1_0066_010}};
	\node [image,right=\padding]                   (result1-depth) at (result1-ods-r.east)       {\subfig{\gcy/output_depth_video1_grandcanyonsequence1_0066_010}};
	
	%% Column 1 :: alpha
	\node [image,below=13.5pt]    (result1-alpha1) at (result1-ods-r.south)  {\subfig{\gcy/mpi_alpha_16}};
	\node [image,below=\padding]  (result1-alpha2) at (result1-alpha1.south) {\subfig{\gcy/mpi_alpha_10}};
	\node [image,below=\padding]  (result1-alpha3) at (result1-alpha2.south) {\subfig{\gcy/mpi_alpha_03}};
	
	%% Column 2 :: blending weights
	\node [image,below=13.5pt]    (result1-blend1) at (result1-ods-l.south)  {\subfig{\gcy/cweight_alphamult_016}};
	\node [image,below=\padding]  (result1-blend2) at (result1-blend1.south) {\subfig{\gcy/cweight_alphamult_010}};
	\node [image,below=\padding]  (result1-blend3) at (result1-blend2.south) {\subfig{\gcy/cweight_alphamult_003}};
	
	%% Column 3 :: MSIs
	\node [image,below=13.5pt]    (result1-msi1) at (result1-depth.south) {\subfig{\gcy/msi_rgblayer_016}};
	\node [image,below=\padding]  (result1-msi2) at (result1-msi1.south)  {\subfig{\gcy/msi_rgblayer_010}};
	\node [image,below=\padding]  (result1-msi3) at (result1-msi2.south)  {\subfig{\gcy/msi_rgblayer_003}};


	%% Labels %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\foreach \result in {1}
	{
		\node [collabel] at (result\result-ods-l.north)  {Left ODS input};
		\node [collabel] at (result\result-ods-r.north)  {Right ODS input};
		\node [collabel] at (result\result-depth.north)  {Pseudo-disparity};
		\node [collabel] at (result\result-alpha1.north) {Alpha maps};
		\node [collabel] at (result\result-blend1.north) {Blending weights};
		\node [collabel] at (result\result-msi1.north)   {Multi-sphere image};
	}
	
	\end{tikzpicture}
	\end{center}
	\vspace{-0.50cm}
	% We need two center environments because, for some reason, '\centering' or a single center environment does not produce the right result.
	\begin{center}
	%
	\newcommand{\imgsize}{0.38\linewidth}
	One IPD --- \emph{Left:} Ours. \emph{Right:} Double-plane-sweep perspective baseline.\\
	\includegraphics[width=\imgsize]{./figures/\gcy/output_tgt_video_box3_grandcanyon1_0065_010.png}
	\includegraphics[width=\imgsize]{./figures/\gcyBaseline/output_tgt_video_box3_grandcanyon1_0065_010.png} \\
	Three IPD \\
	\includegraphics[width=\imgsize]{./figures/\gcy/output_tgt_video_box7_grandcanyon1_0065_010.png}
	\includegraphics[width=\imgsize]{./figures/\gcyBaseline/output_tgt_video_box7_grandcanyon1_0065_010.png} \\
	Five IPD \\
	\includegraphics[width=\imgsize]{./figures/\gcy/output_tgt_video_box11_grandcanyon1_0065_010.png}
	\includegraphics[width=\imgsize]{./figures/\gcyBaseline/output_tgt_video_box11_grandcanyon1_0065_010.png} 
	\end{center}
	%
	\vspace{-0.5cm}
	\caption{\label{fig:results3}
		\emph{GrandCanyon} video results. \emph{Top:} Inferred MSI representation. \emph{Bottom:} Inference for low-resolution (640$\times$480) MSI representation for comparison on spherical images (not our high-res real-time perspective VR view).
		We compare these to the baseline double-plane-sweep method.\protect\linebreak
		From left to right, top to bottom:
        For predicted blending weights, red = left ODS and blue = right ODS;
		for predicted alpha maps, black = transparent and white = opaque.
		The blending weight, alpha maps, and MSI layers are picked as single layers at the near, mid, and far extends of the scene; content exists across all layers to produce the final result.
	}
\end{figure*}

==> src/4-fig-whitehouse1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Image results - Scene 2 White House 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[tp]
	
	\newcommand{\resultDir}{/novel-view-sequence/whitehouse/}
	\newcommand{\baselineDir}{\resultDir/doubleplane-odsods}
	\newcommand{\whitehouseOneIPD}{\resultDir/video1_box_puppy_0150_010/}
    \newcommand{\whitehouseThreeIPD}{\resultDir/video1_box3puppy_0150_010/}
    \newcommand{\whitehouseFiveIPD}{\resultDir/video1_box5puppy_0150_010/}
    \newcommand{\whitehouseBaselineOneIPD}{\baselineDir/video1_box3puppy_0150_010/}
    \newcommand{\whitehouseBaselineThreeIPD}{\baselineDir/video1_box3puppy_0150_010/}
    \newcommand{\whitehouseBaselineFiveIPD}{\baselineDir/video1_box5puppy_0150_010/}
	
	\begin{center}
	\begin{tikzpicture}[
	image/.style={inner sep=0pt, outer sep=0pt},
	collabel/.style={above=9pt, anchor=north, inner ysep=0pt, scale=0.8, align=center},
	rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
	subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
	arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
	]

	\def\padding{0.005\linewidth}
	\newcommand{\subfig}[2][0px 0px 0px 0px]{\includegraphics[width=0.25\linewidth, trim=#1, clip]{figures/#2.png}}
	\newcommand{\subbig}[2][0px 0px 0px 0px]{\includegraphics[width=0.49\linewidth, height=0.3675\linewidth, trim=#1, clip]{figures/#2.png}}
	
	%% Result 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%% Top row :: ODS input + pseudodepth + new view
	\node [image,below=20pt]                       (result1-ods-l) at (0, 0)                     {\subfig{\resultDir/ref_image_video1_whitehouse_0212_010}};
	\node [image,right=\padding]                   (result1-ods-r) at (result1-ods-l.east)       {\subfig{\resultDir/src_image_video1_whitehouse_0212_010}};
	\node [image,right=\padding]                   (result1-depth) at (result1-ods-r.east)       {\subfig{\resultDir/output_depth_video1_whitehouse_0212_010}};

	%% Column 1 :: alpha
	\node [image,below=13.5pt]    (result1-alpha1) at (result1-ods-r.south)  {\subfig{\resultDir/mpi_alpha_31}};
	\node [image,below=\padding]  (result1-alpha2) at (result1-alpha1.south) {\subfig{\resultDir/mpi_alpha_09}};
	\node [image,below=\padding]  (result1-alpha3) at (result1-alpha2.south) {\subfig{\resultDir/mpi_alpha_03}};
	
	%% Column 2 :: blending weights
	\node [image,below=13.5pt]    (result1-blend1) at (result1-ods-l.south)  {\subfig{\resultDir/cweight_alphamult_031}};
	\node [image,below=\padding]  (result1-blend2) at (result1-blend1.south) {\subfig{\resultDir/cweight_alphamult_009}};
	\node [image,below=\padding]  (result1-blend3) at (result1-blend2.south) {\subfig{\resultDir/cweight_alphamult_003}};
	
	%% Column 3 :: MSIs
	\node [image,below=13.5pt]    (result1-msi1) at (result1-depth.south) {\subfig{\resultDir/msi_rgblayer_031}};
	\node [image,below=\padding]  (result1-msi2) at (result1-msi1.south)  {\subfig{\resultDir/msi_rgblayer_009}};
	\node [image,below=\padding]  (result1-msi3) at (result1-msi2.south)  {\subfig{\resultDir/msi_rgblayer_003}};


	%% Labels %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\foreach \result in {1}
	{
		\node [collabel] at (result\result-ods-l.north)  {Left ODS input};
		\node [collabel] at (result\result-ods-r.north)  {Right ODS input};
		\node [collabel] at (result\result-depth.north)  {Pseudo-disparity};
		\node [collabel] at (result\result-alpha1.north) {Alpha maps};
		\node [collabel] at (result\result-blend1.north) {Blending weights};
		\node [collabel] at (result\result-msi1.north)   {Multi-sphere image};
	}
	
	\end{tikzpicture}%
	\end{center}
	%
	\vspace{-0.50cm}
	\begin{center}
	\newcommand{\imgsize}{0.38\linewidth}
	One IPD --- \emph{Left:} Ours. \emph{Right:} Double-plane-sweep perspective baseline.\\
	\includegraphics[width=\imgsize]{./figures/\resultDir/output_tgt_video1_whitehouse_0212_010.png}
	\includegraphics[width=\imgsize]{./figures/\baselineDir/output_tgt_video1_whitehouse_0212_010.png} \\
	Three IPD \\
	\includegraphics[width=\imgsize]{./figures/\resultDir/output_tgt_video1_threeipdwhitehouse_0212_010.png}
	\includegraphics[width=\imgsize]{./figures/\baselineDir/output_tgt_video1_threeipdwhitehouse_0212_010.png} \\
	Five IPD \\
	\includegraphics[width=\imgsize]{./figures/\resultDir/output_tgt_video1_fiveipdwhitehouse_0212_010.png}
	\includegraphics[width=\imgsize]{./figures/\baselineDir/output_tgt_video1_fiveipdwhitehouse_0212_010.png}
	\end{center}
	\vspace{-0.5cm}
	\caption{\label{fig:results2}
		\emph{Whitehouse} video results. \emph{Top:} Inferred MSI representation. \emph{Bottom:} Inference for low-resolution (640$\times$480) MSI representation for comparison on spherical images (not our high-res real-time perspective VR view).
		We compare these to the baseline double-plane-sweep method.\protect\linebreak
		From left to right, top to bottom:
        For predicted blending weights, red = left ODS and blue = right ODS;
		for predicted alpha maps, black = transparent and white = opaque.
		The blending weight, alpha maps, and MSI layers are picked as single layers at the near, mid, and far extends of the scene; content exists across all layers to produce the final result.
	}
\end{figure*}
